Mass Modeling and Kinematics of Galaxy Clusters in Modified Gravity

The chameleon screening mechanism has been constrained many a time using dynamic and kinematic galaxy cluster observables. Current constraints are, however, insensitive to different mass components within galaxy clusters and have been mainly focused on a single mass density profile, the Navarro-Frenk-While mass density model. In this work, we extend the study of the Chameleon screening mechanism in galaxy clusters by considering a series of mass density models, namely: generalized-Navarro-Frenk-While, b-Navarro-Frenk-While, Burket, Isothermal and Einasto. The coupling strength ($\beta$) and asymptotic value of the chameleon field ($\phi_\infty$) are constrained by using kinematics analyses of simulated galaxy clusters, generated both assuming General Relativity and a strong chameleon scenario. By implementing a Bayesian analysis we comprehensively show that the biases introduced due to an incorrect assumption of the mass model are minimal. Similarly, we also demonstrate that a spurious detection of evidence for modifications to gravity is highly unlikely when utilizing the kinematics of galaxy clusters.

==> table.tex <==
\begin{table*}[]
    \centering
     \caption{two-$\sigma$ constraints on the modified gravity parameters  $\phi_2 $,
      $\mathcal{Q}_2$  obtained from the \textsc{MG-MAMPOSSt} 
     fit of two synthetic clusters generated
      in a Chameleon universe with $\phi_2 = 0.65$, 
     $\mathcal{Q}_2 = 0.5$. The first six rows refer to a cluster which true
     mass density follows a Burkert profile, the last six rows to a cluster
     generated assuming a NFW profile. We adopt different mass density models in the fit.}
\begin{tabular}
    {c c | c c  }
    \toprule
    $\rho(r)$ model & fitting model & $\phi_2 $ & $\mathcal{Q}_2$ \\
    \midrule
    \\
    Bur & Bur & $0.47^{+0.14 }_{-0.16}$ & $0.67^{+0.33 }_{-0.22}$ \\
    Bur & NFW & $0.46^{+0.16 }_{-0.17}$ & $0.65^{+0.35 }_{-0.20}$ \\
    Bur & Her & $0.50^{+0.15 }_{-0.15}$ & $0.60^{+0.40 }_{-0.20}$ \\
    Bur & gNFW ($\gamma = 1.2$) & $0.51^{+0.11 }_{-0.11}$ & $0.58^{+0.42 }_{-0.32}$ \\
    Bur & Iso & $0.57^{+0.14 }_{-0.14}$ & $0.57^{+0.41 }_{-0.28}$ \\
    Bur & Ein ($m=2$) & $0.52^{+0.15 }_{-0.15}$ & $0.57^{+0.43 }_{-0.22}$ \\
    \midrule
    NFW & Bur & $0.49^{+0.18 }_{-0.16}$ & $0.68^{+0.32 }_{-0.31}$ \\
    NFW & NFW & $0.46^{+0.18 }_{-0.17}$ & $0.71^{+0.29 }_{-0.30}$ \\
    NFW & Her & $0.48^{+0.18 }_{-0.16}$ & $0.73^{+0.27 }_{-0.41}$ \\
    NFW & gNFW ($\gamma = 1.2$) & $0.47^{+0.12 }_{-0.12}$ & $0.62^{+0.38 }_{-0.45}$ \\
    NFW & Iso & $0.58^{+0.16 }_{-0.14}$ & $0.61^{+0.39 }_{-0.34}$ \\
    NFW & Ein ($m=2$) & $0.54^{+0.28 }_{-0.20}$ & $0.57^{+0.43 }_{-0.42}$ \\
   \end{tabular}

\end{table*}

We found that possible systematic effects due to wrong mass modelling
does not produce any noticeable effect in the distribution of the chameleon parameters,
given reliable statistical uncertainties based on current imaging and spectroscopic surveys.
 
Howeverf, it is worth to quantify the amount of the systematic shift due to the wrong choice of the 
mass model in a ideal situation where the statistical uncertainties
are drastically reduced. To do that, we generate a pps with more than 10000 particles 
following a NFW mass profile in GR, and we further 
assume a perfect knowledge of the parameters $r_{200}$ and $r_\text{s}$ (i.e. 
an infinitely precise prior). One can think to this case as a sort of sta

